Evaluating Protein Transfer Learning with TAPE

Protein modeling is an increasingly popular area of machine learning research. Semi-supervised learning has emerged as an important paradigm in protein modeling due to the high cost of acquiring supervised protein labels, but the current literature is fragmented when it comes to datasets and standardized evaluation techniques. To facilitate progress in this field, we introduce the Tasks Assessing Protein Embeddings (TAPE), a set of five biologically relevant semi-supervised learning tasks spread across different domains of protein biology. We curate tasks into specific training, validation, and test splits to ensure that each task tests biologically relevant generalization that transfers to real-life scenarios. We benchmark a range of approaches to semi-supervised protein representation learning, which span recent work as well as canonical sequence learning techniques. We find that self-supervised pretraining is helpful for almost all models on all tasks, more than doubling performance in some cases. Despite this increase, in several cases features learned by self-supervised pretraining still lag behind features extracted by state-of-the-art non-neural techniques. This gap in performance suggests a huge opportunity for innovative architecture design and improved modeling paradigms that better capture the signal in biological sequences. TAPE will help the machine learning community focus effort on scientifically relevant problems. Toward this end, all data and code used to run these experiments are available at https://github.com/songlab-cal/tape.

==> abstract.tex <==
% NOTE: ADDED ABSTRACT TO main.tex for spacing issues - so this file isn't currently used
Protein modeling is an increasingly popular area of machine learning research. Semi-supervised learning has emerged as an important paradigm in protein modeling due to the high cost of acquiring supervised protein labels, but the current literature is fragmented when it comes to datasets and standardized evaluation techniques.
To facilitate progress in this field, we introduce the Tasks Assessing Protein Embeddings (\benchmarkName), a set of five biologically relevant semi-supervised learning tasks spread across different domains of protein biology. 
We curate tasks into specific training, validation, and test splits to ensure that each task tests biologically relevant generalization that transfers to real-life scenarios.
We benchmark a range of approaches to semi-supervised protein representation learning, which span recent work as well as canonical sequence learning techniques. 
We find that self-supervised pretraining is helpful for almost all models on all tasks, more than doubling performance in some cases. 
Despite this increase, in several cases features learned by self-supervised pretraining still lag behind features extracted by state-of-the-art  non-neural techniques. This gap in performance suggests a huge opportunity for innovative architecture design and improved modeling paradigms that better capture the signal in biological sequences. \benchmarkName will help the machine learning community focus effort on scientifically relevant problems. 
Toward this end, all data and code used to run these experiments are available at \url{https://github.com/songlab-cal/tape}.

% \pa{it'd be good for the abstract to explicitly allude to setting up the benchmark in a maximally accessible way to ML researchers, with train / test splits that have biological relevance, such that improving on the benchmark is directly scientifically relevant}

% \rocky{Is it worth to also briefly motivate semi-supervised learning in the abstract (due to high costs to acquire labels)?}

==> using_tape.tex <==
\section{Using \benchmarkName}
\label{sec:guidelines}

\paragraph{Data} Both raw data and TFRecords files are available for all \benchmarkName tasks at the website. For each task we provide training, validation, and test sets.

It takes considerable experimental and computational resources to produce each dataset in \benchmarkName. Out of respect for this, we insist that anyone using \benchmarkName cite and describe all used dataset components in their paper. To make this easy, we provide a BibTeX file with all dataset citations on the \benchmarkName website, and descriptions of each task are provided above in Section \ref{sec:datasets}. 

\paragraph{Model Availability} For all five models reported in this paper, we provide weights for the pretrained model in the \benchmarkName repository. We further provide code for easily running any task/model pair to enable reproduction of numbers reported in this work.

\paragraph{Leaderboard} We currently do not have a formal leaderboard for \benchmarkName, but we will maintain a table of self-reported top results on the \benchmarkName website that we will keep updated.



